Filter Pruning by Switching to Neighboring CNNs with Good Attributes

Filter pruning is effective to reduce the computational costs of neural networks. Existing methods show that updating the previous pruned filter would enable large model capacity and achieve better performance. However, during the iterative pruning process, even if the network weights are updated to new values, the pruning criterion remains the same. In addition, when evaluating the filter importance, only the magnitude information of the filters is considered. However, in neural networks, filters do not work individually, but they would affect other filters. As a result, the magnitude information of each filter, which merely reflects the information of an individual filter itself, is not enough to judge the filter importance. To solve the above problems, we propose Meta-attribute-based Filter Pruning (MFP). First, to expand the existing magnitude information based pruning criteria, we introduce a new set of criteria to consider the geometric distance of filters. Additionally, to explicitly assess the current state of the network, we adaptively select the most suitable criteria for pruning via a meta-attribute, a property of the neural network at the current state. Experiments on two image classification benchmarks validate our method. For ResNet-50 on ILSVRC-2012, we could reduce more than 50% FLOPs with only 0.44% top-5 accuracy loss.

==> table/table6_time.tex <==

\newcolumntype{N}{>{\centering\arraybackslash}m{0.5in}}


\begin{table}[ht]
\small
\setlength{\tabcolsep}{0.3em}
\begin{center}
\color{red}\begin{tabular}{ N N N N c c  c c   }
\toprule
\multicolumn{5}{c}{Filter Ranking Methods} \\  \cmidrule(r){1-5}
  \multicolumn{2}{c}{Magnitude (\Eqref{eq:p-norm2})} & \multicolumn{2}{c}{Geomotric (\Eqref{eq:Minkowski})} & \multirow{2}{*}{Pearson} & Time & Acc.(\%)    
 \\
 \cmidrule(r){1-2}\cmidrule(r){3-4} 
 p=1 &p=2&q=1&q=2\\
        \cmidrule(r){1-8} 
         
\cmark  & \cmark &        &        &        &           \\
\cmark  & \cmark & \cmark &        &        &         \\
\cmark  & \cmark & \cmark & \cmark &        &           \\
\cmark  & \cmark & \cmark & \cmark & \cmark &           \\
%       &        &        &        &        & \cmark  \\


\bottomrule
\end{tabular}
\end{center}
\caption{
\RR{Accuracy of pruning pre-trained ResNet-110 on CIFAR-10 regarding different execution time. Execution time would increase as filter ranking methods increase.}
}
\label{table:time}
\end{table}


 
